Beyond Negative Transfer: Disentangled Preference-Guided Diffusion for Cross-Domain Sequential Recommendation

Cross-Domain Sequential Recommendation (CDSR) leverages user behaviors across domains to enhance recommendation quality. However, naive aggregation of sequential signals can introduce conflicting domain-specific preferences, leading to negative transfer. While Sequential Recommendation (SR) already suffers from noisy behaviors such as misclicks and impulsive actions, CDSR further amplifies this issue due to domain heterogeneity arising from diverse item types and user intents. The core challenge is disentangling three intertwined signals: domain-invariant preferences, domain-specific preferences, and noise. Diffusion Models (DMs) offer a generative denoising framework well-suited for disentangling complex user preferences and enhancing robustness to noise. Their iterative refinement process enables gradual denoising, making them effective at capturing subtle preference signals. However, existing applications in recommendation face notable limitations: sequential DMs often conflate shared and domain-specific preferences, while cross-domain collaborative filtering DMs neglect temporal dynamics, limiting their ability to model evolving user preferences. To bridge these gaps, we propose \textbf{DPG-Diff}, a novel Disentangled Preference-Guided Diffusion Model, the first diffusion-based approach tailored for CDSR, to or best knowledge. DPG-Diff decomposes user preferences into domain-invariant and domain-specific components, which jointly guide the reverse diffusion process. This disentangled guidance enables robust cross-domain knowledge transfer, mitigates negative transfer, and filters sequential noise. Extensive experiments on real-world datasets demonstrate that DPG-Diff consistently outperforms state-of-the-art baselines across multiple metrics.

==> Fig/elbo.tex <==
 This is typically achieved by optimizing the \textbf{Evidence Lower Bound (ELBO)}:
\begin{align*}
\small
\mathbb{E}[-\log p_{\theta}(x)] 
&\leq \mathbb{E}_q \left[ -\log p(x_T) - \sum_{t=1}^{T} \log \frac{p_{\theta}(x_{t-1}|x_t)}{q(x_{t-1}|x_t)} \right] \\
&= \mathbb{E}_q \Big[ D_{\text{KL}}(q(x_T|x) \,\|\, p(x_T)) 
- \log p_{\theta}(x|x_1) \nonumber \\
&\quad + \sum_{t=2}^{T} D_{\text{KL}}(q(x_{t-1}|x_t, x) \,\|\, p_{\theta}(x_{t-1}|x_t)) \Big]
\end{align*}

In this decomposition:
\begin{itemize}
    \item \( L_T = D_{\text{KL}}(q(x_T|x) \,\|\, p(x_T)) \): KL divergence between the terminal noisy distribution and the prior (a constant, often ignored during optimization),
    \item \( L_0 = -\log p_{\theta}(x|x_1) \): reconstruction loss at final step,
    \item \( L_t = D_{\text{KL}}(q(x_{t-1}|x_t, x) \,\|\, p_{\theta}(x_{t-1}|x_t)) \): step-wise KL divergence for each intermediate transition.
\end{itemize}
